Adversarial Robustness of Deep Neural Networks: A Survey from a Formal Verification Perspective

Neural networks have been widely applied in security applications such as spam and phishing detection, intrusion prevention, and malware detection. This black-box method, however, often has uncertainty and poor explainability in applications. Furthermore, neural networks themselves are often vulnerable to adversarial attacks. For those reasons, there is a high demand for trustworthy and rigorous methods to verify the robustness of neural network models. Adversarial robustness, which concerns the reliability of a neural network when dealing with maliciously manipulated inputs, is one of the hottest topics in security and machine learning. In this work, we survey existing literature in adversarial robustness verification for neural networks and collect 39 diversified research works across machine learning, security, and software engineering domains. We systematically analyze their approaches, including how robustness is formulated, what verification techniques are used, and the strengths and limitations of each technique. We provide a taxonomy from a formal verification perspective for a comprehensive understanding of this topic. We classify the existing techniques based on property specification, problem reduction, and reasoning strategies. We also demonstrate representative techniques that have been applied in existing studies with a sample model. Finally, we discuss open questions for future research.

==> sections/classification_table.tex <==

\begin{table*}
	\begin{center}
		
	\caption{\label{tab:table-classification} Classification of related works according to the reduction approaches and reasoning strategies}
	% Config the row spacing
	\def\arraystretch{1.25}
	% Config the column spacing
	\setlength{\tabcolsep}{3pt}
	\setcounter{rownumber}{0}
	\begin{tabular}{lll|ccccc|ccccc}
		\hline
		\multirow{2}{*}{\textbf{No.}} & \multirow{2}{*}{\textbf{\makecell[l]{Authorship, \\Year \& Reference}}} & \multirow{2}{*}{\textbf{Tool (if any)}} & \multicolumn{5}{l|}{\textbf{Reduction\textsuperscript{1}}} & \multicolumn{5}{l}{\textbf{Reasoning Strategies\textsuperscript{2}}}  \\\cline{4-13}
		& & & \textbf{SAT/LP} & \textbf{MILP} & \textbf{DISC} & \textbf{AI} & \textbf{Others} & \textbf{CR} & \textbf{MO} & \textbf{IA} & \textbf{LA} & \textbf{IR}\\\hline

		\refstepcounter{rownumber}\therownumber & Pulina \& Tacchella, 2010~\cite{pulina2010abstraction} 		& \textsc{neVer}	& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc\\ 
		\refstepcounter{rownumber}\therownumber & Scheibler \textit{et al.}, 2015~\cite{scheibler2015towards} 			& \emptycirc 				& \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc &\fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Bastani \textit{et al.}, 2016	\cite{bastani2016measuring}			& \emptycirc 				& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Carlini \& Wagner, 2017~\cite{carlini2017towards} 			& \emptycirc			 	& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Cheng \textit{et al.}, 2017~\cite{cheng2017maximum}					& \emptycirc 				& \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc\\

		\refstepcounter{rownumber}\therownumber & Ehler, 2017~\cite{ehlers2017formal}							& \textsc{Planet}	& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Huang \textit{et al.}, 2017~\cite{huang2017safety}					& \textsc{DLV}		& \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Katz \textit{et al.}, 2017	\cite{katz2017reluplex}					& \textsc{Reluplex}	& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Lomuscio \& Maganti, 2017~\cite{lomuscio2017approach}		& \emptycirc 				& \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Wong \& Kolter, 2017~\cite{wong2018provable}				& \emptycirc 				& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc\\ 

		\refstepcounter{rownumber}\therownumber & Dutta \textit{et al.}, 2018~\cite{dutta2018output}					& \textsc{Sherlock}	& \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Dvijotham \textit{et al.}, 2018~\cite{dvijotham2018dual}			& \emptycirc 				& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Fischetti \& Jo, 2018	\cite{fischetti2019deep}			& \emptycirc 				& \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Gehr \textit{et al.}, 2018~\cite{gehr2018ai2}						& \textsc{AI2}		& \emptycirc & \emptycirc & \emptycirc & \fullcirc& \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Raghunathan \textit{et al.}, 2018~\cite{raghunathan2018certified}	& \emptycirc 				& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc\\ 

		\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2018~\cite{singh2018fast} 					& \textsc{DeepZ}	& \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Wang \textit{et al.}, 2018~\cite{wang2018formal}					& \textsc{ReluVal}	& \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc\\ 
		\refstepcounter{rownumber}\therownumber & Wang \textit{et al.}, 2018	\cite{wang2018efficient} 				& \textsc{Neurify}	& \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc \\ 
		\refstepcounter{rownumber}\therownumber & Weng \textit{et al.}, 2018	\cite{weng2018towards}					& \textsc{Fast-Lin}, \textsc{Fast-Lip}	& \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Xiang \textit{et al.}, 2018~\cite{xiang2018output} 					& \emptycirc 				& \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc\\ 

		\refstepcounter{rownumber}\therownumber & Zhang \textit{et al.}, 2018~\cite{zhang2018efficient}				& \textsc{CROWN}	& \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Katz \textit{et al.}, 2019	\cite{katz2019marabou}					& \textsc{Marabou}	& \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Tjeng \textit{et al.}, 2019~\cite{tjeng2019evaluating}				& \textsc{MIPVerify}& \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \emptycirc\\ 
		\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2019~\cite{singh2019abstract} 				& \textsc{DeepPoly}	& \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc\\ 
		\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2019~\cite{singh2019boosting}				& \textsc{RefineZono}& \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc\\ 

		\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2019~\cite{singh2019beyond}					& \textsc{kPoly}	& \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc & \fullcirc & \fullcirc \\ 
		\refstepcounter{rownumber}\therownumber & Yisrael \textit{et al.}, 2019~\cite{yisrael2019abstraction} 		& \emptycirc 				& \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \emptycirc & \emptycirc & \fullcirc & \emptycirc & \fullcirc \\ 
		\hline
	\end{tabular}
	
	\end{center}

	\textsuperscript{1} Reduction approaches are classified into five classes as shown in table, where ``SAT/LP'' stands for SAT/LP encoding, ``MILP'' stands for MILP encoding, ``DISC'' stands for discretization and ``AI'' stands for abstract interpretation. The checkmark symbol (\fullcirc) indicates the research work (row) has applied the specific reduction approach (column), otherwise shown as (\emptycirc).
	\vspace{5pt}
	
	\textsuperscript{2} Reasoning strategies are classified into five classes as shown in table, where ``CR'' stands for constraint reasoning, ``MO'' stands for mathematical optimization, ``IA'' stands for interval arithmetic, ``LA'' stands for linear approximation and ``IR'' stands for iterative refinement. The checkmark symbol (\fullcirc) indicates the research work (row) has applied the specific reasoning strategy (column), otherwise shown as (\emptycirc).
\end{table*}

==> sections/deprecated.tex <==
%%%%%%%%%%%%%%%%%%
% properties.tex %
%%%%%%%%%%%%%%%%%%

%---------------------------------------------------------%
% End of the 1st paragraph, before going into subsections %
%---------------------------------------------------------%

% A property $\mathcal{P}$ can be either a \textit{model-specified} character to satisfy certain requirement, or a \textit{general} character that is applicable to any neural network models. The former one is usually used to formalized the functional requirement of a neural network model working as a component within a system. Those properties are converted from quantitative constraints that captured from the system-level specification, and treated as mandatory to ensure the entire system can work as desired. Take the autonomous driving system as example, the system is implemented by a number of different neural networks and the output of the system is generalized through collaboration of more than one component models. One possible model-specified property to the vehicle control subsystem could be defined as follows: the moving command could only be given in case that distance between the vehicle and obstacle is less than a threshold value. Unlike the model-specified properties that are only applicable to specified models as a part of bigger system, general properties are used to describe a characteristic that can be universally applied to any neural network model. In the remaining part of this section, we category the most commonly used (general) properties according to their semantic behaviours and then formalise them for the purpose of verification.

%-------------------------------------------------------------%
% In subsection ``fairness'', by the end of the 2nd paragraph %
%-------------------------------------------------------------%

% Some other notions of fairness property also introduce the \textit{expected output}, written as $\bar{Y}$, which is the manual rectification based on the specific input features by removing discrimination factors. Take the loan application processing model as example, in consideration of prevent gender discrimination, the verifier may provide the $\bar{Y}$ values same for 2 applicants' input that share all same input features except gender details, notated as $\left( \bigwedge_{i=1}^{\left| S \right|}{\{}s_a\left[ i \right] \ne s_b\left[ i \right] \right) \land \left( \bigwedge_{j=1}^{\left| U \right|}{u_a\left[ j \right] =u_b\left[ j \right]} \right) \land \bar{y}_1=\bar{y}_2$. 

% End of fairness subsection %

% Yet another latest literature \cite{kusner2017counterfactual} proposed a novel notion of fairness called \textit{counterfactual fairness}. The notion of counterfactual fairness is implemented based on causal models and provides a more rigorous definition on the fairness. In that notion, given individual inputs with different sensitive features, the conclusion of a neural network model is fair or not could not only determined by the output in the actual world, but also determined by taking the counterfactual world settings in the consideration.

%----------------------------%
% In subsection ``coverage'' %
%----------------------------%

\begin{comment}
\subsubsection{Coverage.}

Coverage properties reason the control flow through traces of a neural network, and reveal the utilisation details of specific neurons or traces.
For example, suppose we have a multiple-layer perceptron (MLP) model with ReLU being selected as the activation function. Coverage details could report a percentage of neurons within the entire model that have activation function in \textit{inactive} mode (always output 0 as all possible inputs are negative and therefore be rectified). In that case, advice regarding change of a better activation function could be provided to achieve better performance of the neural network model. 
Similarly, a low percentage of neuron utilization reported by coverage analysis can help in redesigning of neural network structure, for example reduce number of neurons in specific layers, to optimise the computation resource consumption.

The idea of testing coverage property of a neural network model originates from the testing of digital circuit design, and relevant research implies that could help in testing or semi-formal verification of machine learning model in the future despite this type of property has not yet been widely studied \cite{pei2017deepxplore}. 
\end{comment}

%----------------------------------------------%
% In ver 4.0, all properties definition other  %
%   than Robustness and Security are dropped.  %
%----------------------------------------------%

\begin{comment}

\subsection{Fairness}
\label{subsec-fairness}

Fairness is another important property pending to be verified in fields of machine learning application such as \textit{recommendation system} and \textit{decision making}, especially in those neural network models handling sensitive demographic data. 
Unlike robustness, fairness is not merely a machine learning problem, but a comprehensive concept that integrates with statistics and social sciences.
The notion of fairness property has been widely discussed during the past few years in many literature \cite{kusner2017counterfactual,du2020fairness,seshia2018formal}, and as the result, there are various definitions of fairness properties have been made depending on different understanding of fairness issues to be addressed. 

The \textit{sensitive features} from the input data, which is also known as ``protected attributes'', is the key element in defining the fairness property.
For example, in order to prevent discrimination, the gender is usually defined as the sensitive feature in using neural network to perform job recommendation and loan application;
and race is widely classified as sensitive data in the prediction of social security and crime rate. 
To formalize the property, we use notation of $S$ to represent the set of sensitive features, $U$ to represent the set of insensitive (ordinary) features, and then we separate those sensitive features out from the input $X$. Thus the composition of input features could be written as $X=S \cup U$. 
Here we specially remark that an input feature that being defined to be sensitive only makes sense if it is relevant to the output and substantially plays a role in the neural network, in another word not be zero weighted with in the network.

We categorize various definitions of fairness properties into two types, \textit{individual fairness} and \textit{demographic parity}. Literally, individual fairness emphasizes the influence of sensitive features to the individual outputs. A fair neural network model should keep those sensitive features \textit{invariant} in producing the output, and thereby maps those inputs sharing with the same insensitive features to the same output. 
To simplify the problem, here we assume the verification of fairness is perform on only one sensitive feature per time, and the sensitive feature is a binary attribute that only has two possible values. 
Without considering the context of property, the individual fairness is highly similar to the robustness that we recently defined in Definition \ref{def1} as the case where all perturbations are made on a limited group of sensitive features.

\begin{definition}[Individual fairness] \label{def3}
Suppose there is a neural network model that accepts an m-dimension vector as input.
Given two inputs $x_1,x_2\in\mathbb{R}^m$, that have different sensitive feature, $s_1 \ne s_2$ where $s_1,s_2\in\mathbb{R}$, but have exact same insensitive features, written as $u_1 = u_2$ where $u_1,u_2\in\mathbb{R}^{m-1}$. The individual fairness can be defined as:   
\begin{multline*}
\mathcal{P}_3\left( s_1,s_2,u_1,u_2,y_1,y_2 \right) \\
\overset{\mathrm{def}}{=} \left( \bigwedge_{i=1}^{m-1}{u_1\left[ i \right] =u_2\left[ i \right]} \right) \land \left(s_1\ne s_2 \right) \rightarrow \left(y_1=y_2\right)
\end{multline*}
\end{definition}

There is another definition of individual fairness in \cite{kusner2017counterfactual} stating that, on the premise of sensitive features unidentified, a pair of similar input, $x_1 \approx x_2$, should be led to a pair of similar output $y_1 \approx y_2$. This definition is only applicable to the scenario that the input features and output of a model have a wide domain (e.g. income, age) rather than a binary choices. For example, we can assert that monthly income \$4,200 is more similar with \$4,000 rather than \$5,000, but we cannot compare the similarity among male, female or unspecified gender.
To quantify that similarity, a wide choice of similarity functions or the inverse of distance calculation can be adopted. 

\begin{definition}[Individual fairness considering input/output similarity] \label{def4}
Suppose we have a preferred choice of similarity function $sim(u,v)$ that returns a distance evaluation between two input parameters. With all the settings same as definition \ref{def3}, given the predefined maximum distance of two inputs $\Delta_x$ and the maximum tolerant output distance $\Delta_y$, that type of individual fairness could be written as follows: 
\begin{multline*}
\mathcal{P}_4\left( x_1,x_2,y_1,y_2,\Delta _x,\Delta _y \right) \\
\overset{\mathrm{def}}{=} \left(sim\left( x_1,x_2 \right) \le \Delta _x \right) \rightarrow \left(sim\left( y_1,y_2 \right) \le \Delta _y\right)
\end{multline*}
\end{definition}

The other type of fairness property is demographic parity. It is defined at the population level and emphasizing equality of opportunity.
This type of fairness may tolerate unexpected individual result.  
Instead, it is benchmarked by a probability of getting a group of input features independent or invariant to the final decision making.
Due to the concerned target has grown from two individuals ($x_1, x_2$) to the entire population ($X$), the insensitive input features $U=X \setminus S$ will be ignored in the verification (as they are not forced to be same). 
Here we make use of conditional probability in definition of demographic parity fairness.
Let us once again take the example of loan application. The neural network model that takes demographic details of applicants into account is expected to be fair on applicants' gender, and offers equal opportunity to male and female applicants. 
With hypothesis that the percentage of male and female in all applicants are both 50\%, and demographic parity seeks to obtain an approximately equality in conditional possibilities written as $P(Y=yes|S=male) \approx P(Y=yes|S=female) \approx 50\%$.  

\begin{definition}[Fairness as demographic parity] \label{def5}
Assume the output of given neural network model has $n$ distinct values or segments in its range, written as $\left\{y_1,y_2,...,y_n\right\}$, and given a quantitatively small number $\epsilon$ as the bias tolerance.
The demographic parity fairness on sensitive feature $S$ can be formalized as follows:
\begin{multline*}
\mathcal{P}_5\left( S,Y \right) \\
\overset{\mathrm{def}}{=} \bigwedge_{i=1}^n{\left( \left(P\left( y_i|S \right) \ge P\left( S \right) -\epsilon\right) \land \left(P\left( y_i|S \right) \le P\left( S \right) +\epsilon \right) \right)}
\end{multline*}
\end{definition}

\subsection{Monotonicity}
\label{subsec-monotonicity}

Some literature \cite{you2017deep,dvijotham2018dual} mention monotonicity to be preserved in both input and output of machine learning model in specific application scenarios. 
If we go back to the loan application mentioned in the previous subsection, the monotonicity could be used to establish the link between specific input feature, such as applicants' income, to the final output, which could be the recommendation rate of granting the loan, or the credit limit upon approving the application.
This monotonicity should not only be limited to the quantitative relation -- it can be further extended to the order relation.

\begin{definition}[Partial order monotonicity] \label{def6}
Suppose there are two inputs that satisfy a \textit{partial order relation} like $x_1 \preceq_x x_2$, we expect the outputs of the model retain the monotonic character with respect to the same ordering. We define the partial order relation of output as $ \preceq_y$, which may not have to be same as the partial order relation of input. This property can be formalized as follows:
$$
\mathcal{P}_6\left( x_1,x_2,y_1,y_2, \preceq_x, \preceq_y \right) \overset{\mathrm{def}}{=} \left( \left( x_1\preceq_x x_2 \right)\rightarrow \left( y_1\preceq_y y_2 \right)\right) 
$$
\end{definition}


\subsection{Equivalence}
\label{subsec-equivalence} 

Equivalence is another property that commonly verified in application of neural networks. 
It describes a character of a pair of networks taking inputs from the same domain, represented as two functions $f_1$ and $f_2$ respectively, and always generate the same outputs on any input drawn from its domain. 

In \cite{narodytska2018verifying}, two possible scenarios are introduced where the equivalence of neural networks be discussed in practice.
One scenario is \textit{network alteration}. In case a trained network has been modified to form multiple new models for deployment on different devices, and the user wishes the newly formed models, when running together, could still work as same as the original one, especially when dealing with inputs that are not from training set. Another scenario is called \textit{augmentation reordering}. Consider in an application of image recognition where the input images are augmented or preprocessed before being feeding to a network, equivalence could be used to determine if the order of multiple augmentation processes differentiates the final output of the network model. For example, given a image recognition network $f:X\rightarrow Y$ and two data augmentation transformation function, $g_1:X\rightarrow X$ for image flipping, and $g_2:X\rightarrow X$ for image saturation, equivalence among two models compares the outputs obtained from $f \circ g_1  \circ g_2(X)$ and $f \circ g_2  \circ g_1(X)$. 

\begin{definition}[Equivalence of two models] \label{def8} 
Given two models that take input from the same input distribution, written as $f_1:X\rightarrow Y$ and $f_2:X\rightarrow Y$, equivalence of these two model could be defined as follow: 
$$
\mathcal{P}_8\left( X,f_1,f_2 \right) \overset{\mathrm{def}}{=} \bigwedge_{x\in X}{\left( f_1\left( x \right) =f_2\left( x \right) \right)}
$$
\end{definition}

\end{comment}

%%%%%%%%%%%%%%%%%%
% case_study.tex %
%%%%%%%%%%%%%%%%%%

%---------------%
% Replaced text %
%---------------%

\begin{comment}
We perform a case study on 3 works \cite{katz2017reluplex,lomuscio2017approach,singh2019abstract} mentioned in the previous section. We choose these works not just for the purpose to present different approaches in verifying robustness of neural network models, moreover, to reflect the development and trend along the history in this research area. 
The first work \cite{katz2017reluplex} is one of the best known early works in verifying neural network by formal analysis. Moreover, it is, to our knowledge, the first sound and complete work that proposes to encode the neural network models as a LP problem and certifies a property by solving constraints through a SMT solver. Until this moment, \textsc{Reluplex} is still often mentioned and benchmarked in latest publications despite it only works on simple network architecture with ReLU being the only choice of the activation function. In the latter work \cite{lomuscio2017approach}, a novel MILP encoding is proposed to first time makes the verification no longer rely on a SMT solver. Moreover, a complete convex optimization encoding covering ReLU functions lays foundation for the future enhancement through various mathematical optimization theory.  
The last work \cite{singh2019abstract} we studied makes use of abstract-interpretation to over approximate the output of a neural network model amid a known perturbation being added on the input layer. As one of the latest research, it supports more activation functions and more types of networks. Compared with the first work, it greatly improves the scalability issue in verifying neural network and thereby it is capable to verify a larger models in less time.
Next, we briefly introduce the background techniques that inspire and then be used in each work, followed by demonstrating a common sample network (shown in Fig.\ref{fig:sample_nn_encoding}) to illustrate the process of verification. We leave our discussion gained from the case study to the last section of this paper. 
\end{comment}


%%%%%%%%%%%%%
% case1.tex %
%%%%%%%%%%%%%



\begin{comment}
\begin{figure}[t!]
\begin{equation}
\begin{gathered}
$$
\begin{matrix}
\left( x_1\ge -1 \right) \land \left( x_1\le 1 \right) \land \left( x_2\ge -1 \right) \land \left( x_2\le 1 \right)&	\qquad input\,\,constraints\vspace{5pt}\\
\land \left( x_3=x_1+x_2-1 \right) \land \left( x_4=x_1+x_2+1 \right)& 	\\
\color{teal}{\land \left( x_5\ge x_3 \right) \land \left( x_5\le x_3+M\cdot d_3 \right) \land \left( x_5\ge 0 \right) \land \left( x_5\le M\cdot \left( 1-d_3 \right) \right)}& \\
\color{teal}{\land \left( x_6\ge x_4 \right) \land \left( x_6\le x_4+M\cdot d_4 \right) \land \left( x_6\ge 0 \right) \land \left( x_6\le M\cdot \left( 1-d_4 \right) \right)}& \\
\land \left( x_7=-x_5+x_6+2 \right) \land \left( x_8=-x_5+x_6+1 \right)& \qquad network\,\,specification\\
\color{teal}{\land \left( x_9\ge x_7 \right) \land \left( x_9\le x_7+M\cdot d_7 \right) \land \left( x_9\ge 0 \right) \land \left( x_9\le M\cdot \left( 1-d_7 \right) \right)}& \\
\color{teal}{\land \left( x_{10}\ge x_8 \right) \land \left( x_{10}\le x_8+M\cdot d_8 \right) \land \left( x_{10}\ge 0 \right) \land \left( x_{10}\le M\cdot \left( 1-d_8 \right) \right)} & \\
\land \left( x_{11}=x_9+x_{10} \right) \land \left( x_{12}=x_9-x_{10}+1 \right) & \vspace{5pt}\\
\land \left( x_{11}>x_{12} \right)&		\qquad output\,\,constraints\\
\end{matrix}
$$
\end{gathered}
\nonumber
\end{equation}
\caption{CNF obtained through MILP encoding of the sample network with robustness specification}
\label{fig:cnf-milp-encoding}
\end{figure}

Early works mainly encode a multilayer neural network into a list of constraints in linear programming setting, and then make use of a SMT solver to check satisfiability of the constraints set. Linear programming is a technique for the optimization of a linear objective function, subject to linear equality and linear inequality constraints. 

The \textit{simplex algorithm} is one of classical methods to solve the optimization problem of linear programming. 
It transforms the original algebraic form of a linear programming into a \textit{tableau}, with all rows refer to \textit{basic variables} and all columns refer to \textit{non-basic variables}.
At each time a new state of the tableau is formed, the simplex algorithm first checks if the current assignment of variables reach the optimization. If the answer is no, the simplex algorithm will randomly select one non-basic variable which is eligible to update its value and thus move the entire solution closer to the optimization. A pivot operation is then performed to exchange the role between the selected non-basic variable and basic variable with its updated value, and thereby a new tableau is observed and all above operations will be repeated until either the optimization is achieved, or the problem is proved to have no solution.  
The algorithm used by \textsc{Reluplex} is implemented based on a simplex solver for linear programming problem, with additional features to cope with the ReLU operations in neural networks. 
\textsc{Reluplex} conveys the property of a neural network $\mathcal{P}$ as value ranges of input and output variables, and then transforms the specification of that network as a set of linear constraints.
Specifically in the linear programming encoding, each nodes within a neural network model is treated as a variable, and those variables corresponding to the input and output of neural network are assigned with predefined domains according to the property; each transition between nodes from neighbouring layers links to a constraint. The goal is to find if there exists a solution to maintain the tableau into an stable and optimised status without violating the any domain of variables' assignment. 

\begin{figure}[t!]
\begin{equation}
\begin{gathered}
$$
\mathsf{Pivot_1}\,\,\frac{x_i\in \mathcal{B}, \alpha \left( x_i \right) < l\left( x_i \right) , x_j\in slack^+\left( x_i \right)}{T:=pivot\left( T,i,j \right) , \mathcal{B}:=\mathcal{B}\cup \left\{ x_j \right\} \backslash \left\{ x_i \right\}}
\\
\mathsf{Pivot_2}\,\,\frac{x_i\in \mathcal{B}, \alpha \left( x_i \right) > u\left( x_i \right) , x_j\in slack^-\left( x_i \right)}{T:=pivot\left( T,i,j \right) , \mathcal{B}:=\mathcal{B}\cup \left\{ x_j \right\} \backslash \left\{ x_i \right\}}
\\
\mathsf{Update}\,\,\frac{x_j\notin \mathcal{B}, \left( \alpha \left( x_j \right) <l\left( x_j \right) \right) \lor \left( \alpha \left( x_j \right) >u\left( x_j \right) \right) , l\left( x_j \right) \le \alpha \left( x_j \right) +\delta \le u\left( x_j \right)}{\alpha :=update\left( \alpha ,x_j,\delta \right)}
\\
\mathsf{Update}_b\,\,\frac{x_i\notin \mathcal{B},\left< x_i,x_j \right> \in \mathcal{R},\alpha \left( x_j \right) \ne \max \left( 0,\alpha \left( x_i \right) \right) ,\alpha \left( x_j \right) \ge 0}{\alpha :=update\left( \alpha ,x_i,\alpha \left( x_j \right) -\alpha \left( x_i \right) \right)}
\\
\mathsf{Update}_f\,\,\frac{x_j\notin \mathcal{B},\left< x_i,x_j \right> \in \mathcal{R},\alpha \left( x_j \right) \ne \max \left( 0,\alpha \left( x_i \right) \right)}{\alpha :=update\left( \alpha ,x_j,\max \left( 0,\alpha \left( x_i \right) \right) -\alpha \left( x_j \right) \right)}
\\
\mathsf{PivotForRelu}\,\,\frac{x_i\in \mathcal{B},\exists x_l.\left< x_i,x_l \right> \in \mathcal{R}\lor \left< x_l,x_i \right> \in \mathcal{R},x_j\notin \mathcal{B},T_{i,j}\ne 0}{T:=pivot\left( T,i,j \right) ,\mathcal{B}:=\mathcal{B}\cup \left\{ x_j \right\} \backslash \left\{ x_i \right\}}
\\
\mathsf{ReluSplit}\,\,\frac{\left< x_i,x_j \right> \in \mathcal{R},l\left( x_i \right) <0,u\left( x_i \right) >0}{u\left( x_i \right) :=0\,\,\,\,\,\,\,\,l\left( x_i \right) :=0}
\\
\mathsf{ReluSuccess}\,\,\frac{\forall x\in \mathcal{X} .l\left( x \right) \le \alpha \left( x \right) \le u\left( x \right) ,\forall \left< x^b,x^f \right> \in \mathcal{R}.\alpha \left( x^f \right) =\max \left( 0,\alpha \left( x^b \right) \right)}{\mathtt{SAT}}
$$
\end{gathered}
\nonumber
\end{equation}
\caption{Derivation rules for the abstract \textsc{Reluplex} algorithm}
\label{fig:reluplex-algorithm}
\end{figure}

\begin{figure}[t!]
\begin{equation}
\begin{gathered}
$$
slack^+\left( x_i \right) =\left\{ x_j\notin \mathcal{B}\,| \left( T_{i,j}>0\land \alpha \left( x_j \right) <u\left( x_j \right) \right) \lor \left( T_{i,j}<0\land \alpha \left( x_j \right) >l\left( x_j \right) \right) \right\} 
\\
slack^-\left( x_i \right) =\left\{ x_j\notin \mathcal{B}\,| \left( T_{i,j}<0\land \alpha \left( x_j \right) <u\left( x_j \right) \right) \lor \left( T_{i,j}>0\land \alpha \left( x_j \right) >l\left( x_j \right) \right) \right\} 
$$
\end{gathered}
\nonumber
\end{equation}
\caption{Definition of candidate slack variables for a basic variable}
\label{fig:slack_def}
\end{figure}

\subsubsection*{Algorithm Definition.}

The implementation of \textsc{Reluplex} inherits the traditional 3 key tableau operations: \textit{update}, \textit{pivot} and \textit{satisfiability check}. 
As shown in Fig. \ref{fig:reluplex-algorithm}, the title of majority derivative rules are lent from original simplex algorithm with minor change to adapt to ReLU operations.
For example, the updating operation will be performed on a variable not only when its value goes beyond the predefined boundary, but also if it violates a ReLU connection.
The satisfiability check will not return a positive output if either any variable's value is out-of-bound, or any variable from ReLU connection tuples does not comply the rule of ReLU operations. 
In additional, a derivation rule called $\mathsf{ReluSplit}$ is created to achieve \textit{splitting-on-demand} requirement. It is a divide and conquer approach to separate one verification process into a pair, with one assumes the target ReLU function is active and the other one assumes the same ReLU function as inactive. By doing that, it could save lots of time in the case that update operation being constantly performed on the same ReLU transformation during the simplex tableau processing.

Moreover, slack variables are also defined in assisting the simplex operations. In \textsc{Reluplex}, each basic variable has 2 set of slack variables consist of non-basic variables that constitute the expression of it. As shown in Fig. \ref{fig:slack_def}, one slack variable group for a given basic variable $x_b$, written as $slack^+(x_b)$, enlists all its constitutional non-basic variables that are able to update their values to bring increment in assignment of $x_b$ when its value is lower than its defined range. Similarly, the other slack variable group, presented as $slack^-(x_b)$, is composed by its constitutional non-basic variables that are able to decrease their values to offset the surplus of $x_b$ with respect to its defined range of assignment.  

%$$
%\mathsf{Failure}\,\,\frac{x_i\in \mathcal{B}, \left( \alpha \left( x_i \right) <l\left( x_i \right) \land %slack^+\left( x_i \right) =\emptyset \right) \lor \left( \alpha \left( x_i \right) >u\left( x_i \right) \land %slack^-\left( x_i \right) =\emptyset \right)}{\mathtt{UNSAT}}
%$$

%$$
%\mathsf{Success}\,\,\frac{\forall x_i\in \mathcal{X} .l\left( x_i \right) \le \alpha \left( x_i \right) \le u\left( %x_i \right)}{\mathtt{SAT}}
%$$

\subsubsection*{Demonstration.}

Take the sample neural network from \cite{katz2017reluplex} as example, here we would like to show comprehensive and through procedure to verify if the following property, $v_{11}\in\left[0,\,1\right]$ and $v_{31}\in\left[0.5,\,1\right]$, is preserved or not. First of all we extract all the equations (linear and non-linear) from the sample network as shown below:

\begin{equation}
\begin{gathered}
$$
v_{21}^{b}=v_{11},\, v_{22}^{b}=-v_{11}\\
v_{21}^{f}=max\left(0,v_{21}^{b}\right),\, 
v_{22}^{f}=max\left(0,v_{22}^{b}\right)\\
v_{31}=v_{21}^{f}+v_{22}^{f}
$$
\end{gathered}
\nonumber
\end{equation}

Then we introduce 3 new variables $a_1$, $a_2$ and $a_3$ to solve the verification question in simplex way. 
These 3 new variables are included in a set called basic variables $\mathcal{B}$.
The encoding of the sample network is reflected in 3 linear equations of $a_1$, $a_2$ and $a_3$, which are also known as linear constraints to solve a linear optimization question by simplex algorithm. 
The specification of the network, including the set of all variables $\mathcal{X}$, basic variables $\mathcal{B}$ and tuples reflecting ReLU connection $\mathcal{R}$, are given below:

\begin{equation}
\begin{gathered}
$$
\mathcal{X}=\left\{ v_{11},v_{21}^{b},v_{21}^{f},v_{22}^{b},v_{22}^{f},v_{33},a_1,a_2,a_3 \right\} \\ 
\mathcal{B}=\left\{ a_1,a_2,a_3 \right\}\\
\mathcal{R}=\left\{ \left< v_{21}^{b},v_{21}^{f} \right> ,\left< v_{22}^{b},v_{22}^{f} \right> \right\} \\
a_1=-v_{11}+v_{21}^{b},\, 
a_2=v_{11}+v_{22}^{b},\, 
a_3=-v_{21}^{f}-v_{22}^{f}+v_{31}
$$ 
\end{gathered}
\nonumber
\end{equation}


\begin{figure}[t!]
\centering
%\vspace{-5pt}
\includegraphics[width=0.5\linewidth]{images/reluplex-sample-net.png}
\caption{The example 3 layer neural networks given in the \textsc{Reluplex} paper}
\vspace{-5pt}
\label{fig:reluplex-example}
\end{figure}

At the beginning, a tableau has been formed as shown in $T_0$ of Fig.\ref{fig:reluplex-tableau}, where all the variables are assigned with value in 0. The property to be verified $\mathcal{P}:\alpha \left(v_{11}\right) \in \left[0,1\right], \alpha \left(v_{31}\right) \in \left[0.5,1\right]$ is firstly reflected in the lower and upper bounds of corresponding variables, then the remaining value bounds are set with the maximum range in real number domain, according to the input-output specification in the neural network, e.g. the range of the input variable of a ReLU operator is set as $\left[-\infty,+\infty\right]$ and the output variable is set as $\left[0,+\infty\right]$.

First of all, a $\mathsf{ReluSccuess}$ check is carried out on the initial tableau to check if all the variables' value are within its lower and upper bounds, and all the variables involved in ReLU operations are complying the input-output specifications. We find the value of $v_{31}$ is out-of-bound since its value is by default set to 0. 
Here we have to perform an $\mathsf{Update}$ function to assign $v_{31}$ a new value to make it within its value range. The minimum $\delta$ in that $\mathsf{Update}$ operation is 0.5. 

\begin{table}[ht!]
\centering
\caption{The initial tableau}
\label{table:t0}
\vspace{8pt}
{\renewcommand{\arraystretch}{1.3}%
\begin{tabular}{c|rllllll}
\multicolumn{1}{c|}{\makecell{l\ \ \\\ \ $\boxed{\alpha}$\ \ \\\ \ \ \ u}} 
&  & \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 1}} 
& \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0.5\\ \boxed{0}\\ 1}} \\ \hline
% BELOW IS THE 2nd ROW: non-basic variable names
&     & \multicolumn{1}{c}{$v_{11}$}  
& \multicolumn{1}{c}{$v_{21}^b$} 
& \multicolumn{1}{c}{$v_{21}^f$}  
& \multicolumn{1}{c}{$v_{22}^b$} 
& \multicolumn{1}{c}{$v_{22}^f$}  
& \multicolumn{1}{c}{$v_{31}$} \\ \hline
% BELOW IS THE ROW 3-5: basic variables
\multicolumn{1}{c|}{0  $\boxed{0}$ 0}   & $a_1$= & \multicolumn{1}{c}{$-v_{11}$}  & \multicolumn{1}{c}{$+v_{21}^b$} &       &       &       &       \\
\multicolumn{1}{c|}{0  $\boxed{0}$ 0}   & $a_2$= & \multicolumn{1}{c}{$v_{11}$}   &       &       & \multicolumn{1}{c}{$+v_{22}^b$} &       &       \\
\multicolumn{1}{c|}{0  $\boxed{0}$ 0}   & $a_3$= &       &       & \multicolumn{1}{c}{$-v_{21}^f$} &       & \multicolumn{1}{c}{$-v_{22}^f$} & \multicolumn{1}{c}{$+v_{31}$} 
\end{tabular}}
\end{table}

\begin{figure}[t!]
\centering
\vspace{-5pt}
\includegraphics[width=1\linewidth]{images/reluplex-tableau.png}
\caption{The tableau obtained in \textsc{Reluplex} verification}
\vspace{-10pt}
\label{fig:reluplex-tableau}
\end{figure}

As the result, there is one basic variable $a_3$ subsequently affected since the value of its one component has raised by 0.5. 
According to the simplex algorithm, the basic variable could not update its value directly. Instead, we look for an eligible slack variable from $slack^{-} \left(a_3\right)$ to offset the value increment, then pivot the tableau by replacing that basic variable $a_3$ (the third row in $T_0$) with the eligible slack variable $v_{21}^f$ (the third column in $T_0$).

The tableau after performing $\mathsf{Pivot_2}$ is shown in $T_1$ of Fig.\ref{fig:reluplex-tableau}, where the value $v_{21}^f$ has been raised to 0.5. The updated basic variables and corresponding linear constraints are given below:  


\begin{equation}
\begin{gathered}
$$
\mathcal{B}=\left\{ a_1,a_2,v_{21}^f \right\}\\
a_1=-v_{11}+v_{21}^{b},\, 
a_2=v_{11}+v_{22}^{b},\, 
v_{21}^{f}=-v_{22}^{f}+v_{31}-a_3
$$
\end{gathered}
\nonumber
\end{equation}

\begin{table}[ht!]
\centering
\caption{The tableau after the first pivot operation}
\label{table:t1}
\vspace{8pt}
{\renewcommand{\arraystretch}{1.3}%
\begin{tabular}{c|rllllll}
\multicolumn{1}{c|}{\makecell{l\ \ \\\ \ $\boxed{\alpha}$\ \ \\\ \ \ \ u}} 
&  & \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 1}} 
& \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0.5\\ \boxed{0.5}\\ 1}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 0}} \\ \hline
% BELOW IS THE 2nd ROW: non-basic variable names
&     & \multicolumn{1}{c}{$v_{11}$}  
& \multicolumn{1}{c}{$v_{21}^b$}  
& \multicolumn{1}{c}{$v_{22}^b$} 
& \multicolumn{1}{c}{$v_{22}^f$}  
& \multicolumn{1}{c}{$v_{31}$}
& \multicolumn{1}{c}{$a_3$} \\ \hline
% BELOW IS THE ROW 3-5: basic variables
\multicolumn{1}{c|}{0  $\boxed{0}$ 0}   & $a_1$= & \multicolumn{1}{c}{$-v_{11}$}  & \multicolumn{1}{c}{$+v_{21}^b$} &       &       &       &       \\
\multicolumn{1}{c|}{0  $\boxed{0}$ 0}   & $a_2$= & \multicolumn{1}{c}{$v_{11}$}   &       & \multicolumn{1}{c}{$+v_{22}^b$} &  &       &       \\
\multicolumn{1}{c|}{0  $\boxed{0.5}$ $+\infty$}   & $v_{21}^f$= &       &       &  & \multicolumn{1}{c}{$-v_{22}^f$} & \multicolumn{1}{c}{$+v_{31}$} & \multicolumn{1}{c}{$-a_3$}
\end{tabular}}
\end{table}

The next operation to be performed after pivoting the tableau is satisfiability checking.
Same as the  $\mathsf{ReluSccuess}$ operation that is conducted at very beginning, the assignment of all the variables on the current tableau will be checked against their boundaries, and meanwhile those variables involved in ReLU operations will be checked if they comply the corresponding rules. 
In the tableau as shown in $T_1$, we find all the variables are assigned with a value within its lower and upper bounds, however, one of the variable set that reflects a ReLU connection, $\left< v_{21}^{b},v_{21}^{f} \right>$, violates the rule of ReLU operation that $v_{21}^f$ is supposed to be equal to $max \left(0, v_{21}^{b}\right)$.
On the contrary, $v_{21}^f=0$ but $v_{21}^f=0.5$ at this moment. An update operation specifically designed for resolving ReLU connections will be performed in the next step.

Since $v_{21}^f$ is a basic variable in the current tableau, and $v_{21}^b$ is not among basic variables -- thus $v_{21}^b$ is selected to be updated in accordance with derivation rule $\mathsf{Update_b}$, where the offset value $\delta=0.5$ and the candidate non-basic variable from $slack^{-}\left(a_1\right)$ is $v_{11}$, located in the first row in the tableau.
After the updating, the value assigned to $v_{11}$ is raised to 0.5 and another $\mathsf{Pivot_2}$ is performed to replace $a_1$ from the basic variable set by $v_{11}$. The updated set of constraints are given below, and the new tableau after the second pivoting is shown in $T_2$ of Fig.\ref{fig:reluplex-tableau}.

\begin{equation}
\begin{gathered}
$$
\mathcal{B}=\left\{ v_{11},a_2,v_{21}^f \right\}\\
v_{11}=v_{21}^{b}-a_1,\, 
a_2=v_{21}^{b}+v_{22}^{b}-a_1,\, 
v_{21}^{f}=-v_{22}^{f}+v_{31}-a_3
$$
\end{gathered}
\nonumber
\end{equation}

\begin{comment}
\begin{table}[ht!]
\centering
\caption{The tableau after the second pivot operation}
\label{table:t2}
\vspace{8pt}
{\renewcommand{\arraystretch}{1.3}%
\begin{tabular}{c|rllllll}
\multicolumn{1}{c|}{\makecell{l\ \ \\\ \ $\boxed{\alpha}$\ \ \\\ \ \ \ u}} 
&  & \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0.5}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0.5\\ \boxed{0.5}\\ 1}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 0}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 0}} \\ \hline
% BELOW IS THE 2nd ROW: non-basic variable names
&     & \multicolumn{1}{c}{$v_{21}^b$}  
& \multicolumn{1}{c}{$v_{22}^b$} 
& \multicolumn{1}{c}{$v_{22}^f$}  
& \multicolumn{1}{c}{$v_{31}$}
& \multicolumn{1}{c}{$a_1$}  
& \multicolumn{1}{c}{$a_3$} \\ \hline
% BELOW IS THE ROW 3-5: basic variables
\multicolumn{1}{c|}{0  $\boxed{0.5}$ 1}   & $v_{11}$= & \multicolumn{1}{c}{$v_{21}^b$} &       &       &       & \multicolumn{1}{c}{$-a_1$} & \\
\multicolumn{1}{c|}{0  $\boxed{0.5}$ 0}   & $a_2$= & \multicolumn{1}{c}{$v_{21}^b$} & \multicolumn{1}{c}{$+v_{22}^b$} &  &  & \multicolumn{1}{c}{$-a_1$} & \\
\multicolumn{1}{c|}{0  $\boxed{0.5}$ $+\infty$}   & $v_{21}^f$= & & & \multicolumn{1}{c}{$-v_{22}^f$} & \multicolumn{1}{c}{$+v_{31}$} & & \multicolumn{1}{c}{$-a_3$}
\end{tabular}}
\end{table}

A $\mathsf{ReluSeccuss}$ is performed after each time we create a new tableau through pivoting. 
We observe the assignment of $a_2$ violates its value boundary due to the value change of $v_{21}^b$ occurred in the last update operation.
As the result, $v_{22}^b$ is chosen from $slack^{-}\left(a_2\right)$ to offset the superfluous amount in assignment of $a_2$ (i.e. to make $\alpha\left(a_2\right)=0$ again). An $\mathsf{Update}$ on $v_{22}^b$ with $\delta=-0.5$ is carried out and then be followed by a $\mathsf{Pivot_2}$ operation to replace $a_2$ from the basic variables by $v_{22}^b$. 
You can find the tableau after the third pivoting in $T_3$ of Fig.\ref{fig:reluplex-tableau}. 
The updated basic variables and corresponding linear constraints are given below: 

\begin{equation}
\begin{gathered}
$$
\mathcal{B}=\left\{ v_{11},v_{22}^b,v_{21}^f \right\}\\
v_{11}=v_{21}^{b}-a_1,\, 
v_{22}^{b}=-v_{21}^{b}+a_1+a_2,\, 
v_{21}^{f}=-v_{22}^{f}+v_{31}-a_3
$$
\end{gathered}
\nonumber
\end{equation}

\begin{comment}
\begin{table}[ht!]
\centering
\caption{The tableau after the third pivot operation, where the positive outcome of $\mathsf{ReluSccuess}$ is observed}
\label{table:t3}
\vspace{8pt}
{\renewcommand{\arraystretch}{1.3}%
\begin{tabular}{c|rllllll}
\multicolumn{1}{c|}{\makecell{l\ \ \\\ \ $\boxed{\alpha}$\ \ \\\ \ \ \ u}} 
&  & \multicolumn{1}{c}{\makecell{$-\infty$\\ \boxed{0.5}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ $+\infty$}} 
& \multicolumn{1}{c}{\makecell{0.5\\ \boxed{0.5}\\ 1}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 0}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 0}} 
& \multicolumn{1}{c}{\makecell{0\\ \boxed{0}\\ 0}} \\ \hline
% BELOW IS THE 2nd ROW: non-basic variable names
&     & \multicolumn{1}{c}{$v_{21}^b$}   
& \multicolumn{1}{c}{$v_{22}^f$}  
& \multicolumn{1}{c}{$v_{31}$}
& \multicolumn{1}{c}{$a_1$}  
& \multicolumn{1}{c}{$a_2$}
& \multicolumn{1}{c}{$a_3$} \\ \hline
% BELOW IS THE ROW 3-5: basic variables
\multicolumn{1}{c|}{0  $\boxed{0.5}$ 1}   & $v_{11}$= & \multicolumn{1}{c}{$v_{21}^b$} & &       & \multicolumn{1}{c}{$-a_1$} & & \\
\multicolumn{1}{c|}{$-\infty$  $\boxed{-0.5}$ $+\infty$}   & $v_{22}^b$= & \multicolumn{1}{c}{$-v_{21}^b$} & & & \multicolumn{1}{c}{$+a_1$} & \multicolumn{1}{c}{$+a_2$}  & \\
\multicolumn{1}{c|}{0  $\boxed{0.5}$ $+\infty$}   & $v_{21}^f$= & & \multicolumn{1}{c}{$-v_{22}^f$} & \multicolumn{1}{c}{$+v_{31}$} & & &  \multicolumn{1}{c}{$-a_3$} 
\end{tabular}}
\end{table}

In the end, after the third pivot operation performed on the tableau, another $\mathsf{ReluSccuess}$ check is carried out and then a $\mathsf{SAT}$ output is observed -- which means the property $\mathcal{P}$ is successfully verified in the given neural network.

\end{comment}


%%%%%%%%%%%%%
% case2.tex %
%%%%%%%%%%%%%


%----------------------------------%
% Intro of abstract interpretation %
%----------------------------------%

% Depends on the nature of property to be verified, the abstraction could be non-relational or relational to approximate the set of finite or infinite variables, corresponding to a function’s domain and range, during the program execution. \textit{Sign abstraction} and \textit{interval abstraction} are typical non-relational abstraction, which ignore the relationship between the exact value of the input ($X$) and the output ($Y$) of the concrete function but emphasises only one or more specific attributes. 
% On the contrary, relational abstraction, such as \textit{octagonal abstraction} and \textit{polyhedral abstraction}, provides a more precise analysis as it attempts to construct a set of linear polynomial equations or inequations containing the input ($X$) and the output ($Y$) of the concrete function.

\begin{comment}
\begin{figure}[t!]
	\centering
	\vspace{-5pt}
	\includegraphics[width=0.98\linewidth]{images/abstraction_types.png}
	\caption{Abstraction of a set of 2-dimension scattered points in various domain}
	\vspace{-10pt}
	\label{fig:abstractdomain}
\end{figure}
\end{comment}

%--------------------------------------------------%
% Demonstration of DeepPoly on its example network %
%--------------------------------------------------%


\begin{comment}

\subsubsection{Demonstration.}

We borrow the sample offered in the studied paper, which demonstrates a typical MLP feedforward neural network. As shown in the fig.~\ref{fig:samplenn}, there are 4 layers in the given sample neural network, including the input layer, output layer and 2 hidden layers. There are affine operation being placed between each layer in a fully connected manner, besides that, the ReLU operation as the choice of activation function are performed within each neurons on hidden layers, right after the affine operation. In the given sample, the neural network is constructed by 8 neurons, with 6 affine operations and 4 ReLU operations involved. To fully present the abstract transformation occurred in the given sample, 12 variables are defined and indexed in feedforward order. The input of the neural network is assumed to be normalised and the enforced perturbation (i.e. [-1,1]) is presented as the value of the first layer variables, which are $x_1$ and $x_2$ shown in the sample corresponding to 2 input features. 
For the purpose to certify robustness of the sample, we check the specification, namely whether all concrete output values of one neuron are always greater than all concrete output values of the other neuron, i.e.:

\begin{center}
	if $\forall i_1,i_2\in \left[ -1,1 \right] \times \left[ -1,1 \right] ,x_{11}>x_{12}$, or\\
	$\forall i_1,i_2\in \left[ -1,1 \right] \times \left[ -1,1 \right] ,x_{11}<x_{12}$.
\end{center}

where $x_{11}$, $x_{12}$ = $f\left(i_1,i_2\right)$ are the concrete values for variables $x_{11}$ and $x_{12}$ produced by our feedforward neural network $f$ for inputs $i_1$, $i_2$.
To address this question, an addition variable $x_{13}$, is created as $x_{13}=x_{11}-x_{12}$. In that way, if we can show the range of $x_{13}$ is permanently greater than 0 or less than 0, then we can prove that the specification holds in the verified neural network in dealing with perturbations within the range [-1,1].

Due to the limitation of space, we will not present abstraction and deductive concretisation of all nodes in the sample network, but selectively show the deduction and calculation of 2 nodes in the hidden layers $x_{4},\,x_{5}$ as well as the final additional node $x_{13}$. 

Let's start with $x_4$. $x_4$ is the result of an affine operation:

\begin{equation}
\begin{array}{l@{}l}
$$x_4&{}=v_4+\sum_{j\in \text{K}}{\left( w_j\cdot x_j \right)}, \text{where K}=\left[ 1,2 \right] \\
&{}=0 + \left( 1\times x_1 +\left( -1 \right) \times x_2 \right) \\
&{}=x_1-x_2$
$ \nonumber
\end{array}
\end{equation}

According to the rule defined for affine function, we have $a_{4}^{'\le}\left( x \right) =a_{4}^{'\ge}\left( x \right) =x_1-x_2$.

Then both invariants $u$ and $l$ can be computed as follows:

\begin{equation}
\begin{array}{l@{}l}
$$l_{4}^{'}
&{}=v'+\sum_{j\in \left[ k \right]}{\left( \max \left( 0,w_{j}^{'} \right) \cdot a_{j}^{'\le}\left( x \right) +\min \left( w_{j}^{'},0 \right) \cdot a_{j}^{'\ge}\left( x \right) \right)}\\
&{}=a_{1}^{'\le}\left( x \right) -a_{2}^{'\ge}\left( x \right) \\
&{}=-2$$ \nonumber
\end{array}
\end{equation}

\begin{equation}
\begin{array}{l@{}l}
$$u_{4}^{'}
&{}=v'+\sum_{j\in \left[ k \right]}{\left( \max \left( 0,w_{j}^{'} \right) \cdot a_{j}^{'\ge}\left( x \right) +\min \left( w_{j}^{'},0 \right) \cdot a_{j}^{'\le}\left( x \right) \right)}\\&{}=a_{1}^{'\ge}\left( x \right) -a_{2}^{'\le}\left( x \right) \\
&{}=2$$ \nonumber
\end{array}
\end{equation}

To sum up, the transformation of $x_{4}$ in the second layer could be depicted as:

\begin{center}
	$f:x_4\gets x_1-x_2$ s.t. $T_{f}^{\#}\left( \left< a^{\le},a^{\ge},l,u \right> \right) =\left< x_1-x_2,x_1-x_2,-2,2 \right> $
\end{center}

Next, let's look at $x_5$, which is the result of ReLU operation: $x_5=\max \left( 0,x_3 \right) $.
In consideration of invariant bound of the input $x_3$ is [-2, 2], so we can obtain both polyhedral constraints by the case (3) introduced in the previous section, and since $\left| l_3 \right|=\left| u_3 \right|$, we set $\lambda=0$:

\begin{center}
	$$a_{5}^{'\le}\left( x \right) =\lambda \cdot x_3=0$$
	$$a_{5}^{'\ge}\left( x \right) =u_3\frac{\left( x_3-l_3 \right)}{\left( u_3-l_3 \right)}=0.5 \cdot x_3+1$$
	$$l'_{5}=\lambda \cdot l_3=0$$
	$$u'_{5}=u_{3}=2$$
\end{center}

As the result, the transformation of $x_{5}$ could be summarised as:

\begin{center}
	$f:x_5\gets\max \left( 0,x_3 \right)$ s.t. $T_{f}^{\#}\left( \left< a^{\le},a^{\ge},l,u \right> \right) =\left< 0, 0.5 \cdot x_3 + 1,0,2 \right> $
\end{center}

In the end, let's move to the additional variable created to prove robustness of the sample network, $x_{13}$.
For the associated invariant constraints, we have 
$a_{13}^{'\le}\left( x \right) =a_{13}^{'\ge}\left( x \right) =x_{11}-x_{12}$

Next, to obtain the concretisation boundary of $x_{13}$, we calculate the associate constraints $l'_{13}$ and $u'_{13}$. The substitution is performed like below:

\begin{equation}
\begin{array}{l@{}l}
$$b_2\left( x \right) &{}=v'+\sum_{j\in \left[ k \right]}{\left( \max \left( 0,w_{j}^{'} \right) \cdot a_{j}^{'\le}\left( x \right) +\min \left( w_{j}^{'},0 \right) \cdot a_{j}^{'\ge}\left( x \right) \right)}\\
&{}=0+\left( 1\times a_{11}^{'\le}\left( x \right) +0\times a_{12}^{'\le}\left( x \right) \right) +\left( 0\times a_{11}^{'\ge}\left( x \right) +\left( -1 \right) \times a_{12}^{'\ge}\left( x \right) \right) \\
&{}=a_{11}^{'\le}\left( x \right) -a_{12}^{'\ge}\left( x \right) \\
&{}=\left( x_9+x_{10}+1 \right) -x_{10}\\
&{}=1+x_9$$
\end{array} \nonumber
\end{equation}

Here we directly refer to the result $l'_{9}=0$ that shown on Fig.\ref{fig:samplenn}, thereby we have $l'_{13}=1$.

On the other side, we set $c_1\left( x \right) =a_{13}^{'\ge}\left( x \right) $, then the substitution could be performed as below:

\begin{equation}
\begin{array}{l@{}l}
$$c_2\left( x \right) &{}=v'+\sum_{j\in \left[ k \right]}{\left( \max \left( 0,w_{j}^{'} \right) \cdot a_{j}^{'\ge}\left( x \right) +\min \left( w_{j}^{'},0 \right) \cdot a_{j}^{'\le}\left( x \right) \right)}\\
&{}=0+\left( 1\times a_{11}^{'\ge}\left( x \right) +0\times a_{12}^{'\ge}\left( x \right) \right) +\left( 0\times a_{11}^{'\le}\left( x \right) +\left( -1\times a_{12}^{'\le}\left( x \right) \right) \right) \\
&{}=a_{11}^{'\ge}\left( x \right) -a_{12}^{'\le}\left( x \right) \\
&{}=\left( x_9+x_{10}+1 \right) -x_{10}\\
&{}=1+x_9$$
\end{array} \nonumber
\end{equation}

In the same way, we directly refer to the result $u'_{9}=3$ depicted in Fig.\ref{fig:samplenn}, then we obtain $u'_{13}=4$. 

As the concrete bound of $x_{13}$ is [1,4], which is always greater than 0, our analysis concludes that $x_{11}-x_{12}>0$ holds, and the robustness of the given neural network could be proved.

\end{comment}


==> sections/survey_table.tex <==
\afterpage{
	\onecolumn
	\footnotesize
	% Config the row spacing
	\def\arraystretch{1.1}
	% Config the column spacing
	\setlength{\tabcolsep}{2pt}
	\setcounter{rownumber}{0}
	\begin{landscape}
		\begin{longtable}[l]{
				>{\raggedright\arraybackslash}p{0.02\hsize}
				>{\raggedright\arraybackslash}p{0.16\hsize}
				p{0.62\hsize}
				>{\centering\arraybackslash}p{0.08\hsize}
				>{\centering\arraybackslash}p{0.015\hsize}
				>{\centering\arraybackslash}p{0.015\hsize}
				>{\centering\arraybackslash}p{0.015\hsize}
				>{\centering\arraybackslash}p{0.015\hsize}
			}
			\caption{Survey Result of Neural Network Robustness Verification}\label{tab:survey_table} \\ 
			\hline
			\rule{0pt}{1.65\normalbaselineskip} & & & 
			& \multicolumn{3}{c}{\textbf{\makecell[l]{Supported\\Activation\textsuperscript{$\dagger$}}}} 
			& \multirow{2}{*}{\rotatebox{90}{\parbox{1.7cm}{\raggedright\textbf{Completeness\textsuperscript{$\ddagger$}}}}} 
			\\[5pt] \cline{5-7}
			\textbf{No.} & \textbf{\makecell[l]{Authorship, Year,\\Reference \& Name of Tool\\(if any)}}  
			& \textbf{\makecell[l]{Summary of Contribution}}
			& \textbf{\makecell[l]{Supported\\Framework\\ \& Link (if any)}}  
			& \textbf{\rotatebox[origin=c]{90}{\makecell[l]{ReLU}}} 
			& \textbf{\rotatebox[origin=c]{90}{\makecell[l]{\ Sigmoid\ \ }}} 
			& \textbf{\rotatebox[origin=c]{90}{\makecell[l]{Tanh}}} 
			&  \\ [5pt] \hline
			
		
			\endfirsthead	
			\multicolumn{7}{c}%
			{{\tablename\ \thetable{} -- continued from the previous page}} \\ 
			\hline
			\rule{0pt}{1.65\normalbaselineskip} & & & 
			& \multicolumn{3}{c}{\textbf{\makecell[l]{Supported\\Activation\textsuperscript{$\dagger$}}}} 
			& \multirow{2}{*}{\rotatebox{90}{\parbox{1.7cm}{\raggedright\textbf{Completeness\textsuperscript{$\ddagger$}}}}} 
			\\[5pt] \cline{5-7}
			\textbf{No.} & \textbf{\makecell[l]{Authorship, Year,\\Reference \& Name of Tool\\(if any)}}  
			& \textbf{\makecell[l]{Summary of Contribution}}
			& \textbf{\makecell[l]{Supported\\Framework\\ \& Link (if any)}}  
			& \textbf{\rotatebox[origin=c]{90}{\makecell[l]{ReLU}}} 
			& \textbf{\rotatebox[origin=c]{90}{\makecell[l]{\ Sigmoid\ \ }}} 
			& \textbf{\rotatebox[origin=c]{90}{\makecell[l]{Tanh}}} 
			&  \\ [5pt] \hline
			
			\endhead	
			\multicolumn{7}{c}{\makecell[c]{\\Continued on the next page}} \\ \hline
			\endfoot
			\hline 
			\endlastfoot

\refstepcounter{rownumber}\therownumber & Pulina \& Tacchella, 2010~\cite{pulina2010abstraction} \newline \textsc{neVer}					
	& The first work that proposes abstraction in verifying a DNN and introduces a linear approximation algorithm to estimate the interval of Sigmoid outputs. Adopts the idea of CEGAR to mitigate spurious counterexamples.
%	& Poor scalability and precision due to the coarse approximation.& -- 
	& Shark (C++)
	& --	& \checkmark	& --	& --\\ \hline	
\refstepcounter{rownumber}\therownumber & Scheibler \textit{et al.}, 2015~\cite{scheibler2015towards} \newline-- 					
	& Proposes an encoding scheme to reduce MLP models into linear \& non-linear arithmetic formulas and then solve by iSAT.
%	& The encoding is constructed on a specific industrial application rather than general DNN, and is not scalable, too. & -- 
	& Not Specified
	& --	& \checkmark & -- & \checkmark \\ \hline
\refstepcounter{rownumber}\therownumber & Bastani \textit{et al.}, 2016	\cite{bastani2016measuring}	\newline \unofficialname{ILP}
	& Introduces a formal definition of $L_{\infty}$ norm robustness property and proposes a constraint set based encoding of DNN that can be solved by any available LP solver. Proves the non-robustness by under-approximating the propagation caused by adversarial inputs, i.e. the minimum perturbation to make the model misclassify.
%	& The analysis is performed on the basis of selected  counterexamples and focus more on finding adversarial input. & -- 
	& Caffe
	& \checkmark & -- & --	& -- \\ \hline

% Carlini and Wagner's work does not study the formal verification therefore we omit it
%\refstepcounter{rownumber}\therownumber & Carlini \& Wagner, 2017~\cite{carlini2017towards} \newline --				
%	& Reduces a neural network as an LP problem and use Adam optimizer to find the adversarial perturbations.
%	& The work does not propose a general solution for neural network verification. & -- 
%	& \textcolor{red}{Not Specified}
%	& \checkmark & -- & -- & \checkmark\\ \hline

\refstepcounter{rownumber}\therownumber & Cheng \textit{et al.}, 2017~\cite{cheng2017maximum}	\newline \unofficialname{MaxResilience}					
	& Proposes a complete formalization to reduce verification of a neural network with piecewise linear activation functions to an MILP problem in a big-M encoding, and an approximation for arctan function with error bounds.
%	& Poor scalability that only works with NN models with less than 200 neurons. & -- 
	& ConvNetJS
	& \checkmark & -- & --	& \checkmark\textsuperscript{$\S$} \\ \hline
\refstepcounter{rownumber}\therownumber & Ehler, 2017~\cite{ehlers2017formal} \newline \textsc{Planet}		
	& Proposes a novel combination of linear approximation of piecewise linear activation functions and searching over the reduced SAT/LP encoding, and thus reduces the search space for the solving. Benchmarks on different types of solvers, and natively supports Max Pooling for CNN.
%	& Unfavorable performance on large neural network. & \checkmark
	& Caffe %\footnote{\url{https://github.com/progirep/planet}}
	& \checkmark & --	& -- & \checkmark \\ \hline
\refstepcounter{rownumber}\therownumber & Huang \textit{et al.}, 2017~\cite{huang2017safety} \newline \textsc{DLV}
	& Proposes a feedforward analysis that partially based on discretization that reduces the infinite ($L_{1}$ and $L_{2}$ norms) neighborhood of a benign input into a finite set of points, and performs verification by proving the consistent labeling among the benign input and its neighboring data points.
%	& The work does not focus on general verification of property specification with weak guarantees and limitation that only works for  specific L1-norm distortion. & \checkmark
	& Keras \,(Theano)%~\footnote{\url{https://github.com/verideep/dlv}}
	& \checkmark	& --  &  --	& \checkmark\\ \hline
\refstepcounter{rownumber}\therownumber & Katz \textit{et al.}, 2017	\cite{katz2017reluplex}	\newline \textsc{Reluplex}	
	& Proposes a  verification solution by applying divide-and-conquer strategy and solve the LP encoding through simplex algorithm, which first time marking complete verification practical for deep neural network with up to 1000 neurons. Proves DNN verification is NP-complete. Floating point precision and big-M MILP encoding are also discussed.
%	& Incapable to handle larger neural networks due to the limitation of LP encoding, and unsound for floating point arithmetic.. & \checkmark
	& Not Specified (written in C)%~\footnote{\url{ht tps://github.com/guykatzz/ReluplexCav2017}}
	& \checkmark & --	& -- & \checkmark \\ \hline
\refstepcounter{rownumber}\therownumber & Lomuscio \& Maganti, 2017~\cite{lomuscio2017approach}\newline \unofficialname{NSVerify}
	& Proposes a reachability analysis setting for DNN verification that encodes a DNN into an MILP problem and certifies the property specification through a solver. It also takes soundness of floating point arithmetic into account.
%	& Poor scalability that only works with neural network models with up to 3 layers.& -- 
	& Not Specified
	& \checkmark & --	& -- 	& \checkmark \\ \hline
\refstepcounter{rownumber}\therownumber & Wong \& Kolter, 2018~\cite{wong2018provable} \newline \textsc{ConvexAdversarial}%, \unofficialname{ConvDual, LP-Full}		
	& Uses the idea of convex outer adversarial polytope in ReLU DNNs to compute a certified lower bound by linear relaxation of ReLU, and transforming the original LP problem to its dual formulation.
%	& Emphasizes on guiding the training process of robust DNNs rather than robustness verification with scope of perturbation has pre-defined at the input layer. & \checkmark 
	& PyTorch %\footnote{\href{https://github.com/locuslab/convex_adversarial}{https://github.com/locuslab/convex\_adversarial}}
	& \checkmark & --	& -- & --\\ \hline
\refstepcounter{rownumber}\therownumber & Xiang \textit{et al.}, 2017~\cite{xiang2017reachable} \newline \unofficialname{ExactReach}	
	& Proposes safety verification of ReLU neural network through reachable set computation. Given the safe input as a halfspace polytope, it produces the exact bounds of the network's output as another halfspace polytope. The benchmarking costs over 10 minutes to perform verification of a model with seven hidden layers. 
	& MATLAB
	&\checkmark & -- & -- & \checkmark \\ \hline

\refstepcounter{rownumber}\therownumber & Dutta \textit{et al.}, 2018~\cite{dutta2018output}	\newline \textsc{Sherlock}		
	& Encodes a deep neural network into MILP, then relaxes the integer constraints with real values, and proposes an algorithm that iteratively combines traditional MILP solving and local optimization to improve performance and scalability so as to handle DNN with over 6000 neurons.
%	& Limited scalability when handling larger NN models.. & \checkmark
	& Not Specified (written in C++)%~\footnote{\url{https://github.com/verivital/sherlock}}
	 & \checkmark & --	& -- 	& \checkmark \\ \hline
\refstepcounter{rownumber}\therownumber & Dvijotham \textit{et al.}, 2018~\cite{dvijotham2018dual}	\newline  \unofficialname{DeepVerify} or \unofficialname{Duality}					
	& Adopts Lagrangian relaxation to transform the original non-convex optimization encoding of DNN into an unconstrained dual formulation. Supports any activation function that is Lipschitz continuous.
%	& Improves the quality of robustness bound estimation but still comes with poor scalability. & -- 
	& Tensorflow%~\footnote{\url{https://github.com/deepmind/deep-verify}}
	& \checkmark	& \checkmark		& \checkmark			 & --\\ \hline

% Fischetti and Jo's work doesn't formally cover verification, consider to omit it
%\refstepcounter{rownumber}\therownumber & Fischetti \& Jo, 2018	\cite{fischetti2019deep}	\newline  --					
%	& Proposes a 0-1 MILP encoding to reduce a DNN for property verification and reasons through a MILP solver, and implements a \emph{asymmetric bound tightening} mechanism to reduce the search space.
%	& Poor scalability that can only verify a DNN with maximum 100-200 neurons due to the lack of heuristic optimization in its implementation.& -- 
%	& \textcolor{red}{Not Specified}
%	& \checkmark & --	& -- 	& \checkmark\\ \hline
\refstepcounter{rownumber}\therownumber & Raghunathan \textit{et al.}, 2018~\cite{raghunathan2018certified}	\newline  \unofficialname{AdvDefense} or \unofficialname{Certify}					
	& Proposes a semidefinite relaxation to compute the over-approximated bounds at output layer (aka. certificates). It is capable to verify a specific property specification for neural networks with (\textit{only}) one hidden layer, and supports any activation that is piecewise differentiable.
	%	& Poor scalability that this work is limited to NNs with one hidden layer only. & -- 
	& Tensorflow% \footnote{\url{https://worksheets.codalab.org/worksheets/0xa21e794020bb474d8804ec7bc0543f52/}}
	& \checkmark	& \checkmark		& \checkmark	 & --\\ \hline

\refstepcounter{rownumber}\therownumber & Gehr \textit{et al.}, 2018~\cite{gehr2018ai2}	\newline  \textsc{AI2}			
	& Conveys reasoning of DNN in terms of abstract interpretation, and therefore verifies a property specification from interpreting its over-approximation result. Compared with traditional SAT/LP encoding approaches, it achieves much better scalability to prove robustness of similar DNN models. It also discusses trade-off between precision and scalability among different abstract domains, and support of image rotation in the verification through zonotope abstract domain.
%	& Models ReLU as a conditional function and apply joining operations to reason the output rather than applying faster and more efficient linear approximation.& -- 
	& PyTorch \& Tensorflow %\footnote{\url{https://github.com/eth-sri/eran}}
	& \checkmark	& --	& -- & --\\ \hline
\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2018~\cite{singh2018fast} 	\newline  \textsc{DeepZ}		
	& The first work that takes cares of floating point soundness in estimating bounds of neuron output, and proposes linear approximation for various activation functions in the view of abstract interpretation. It further improves the scalability of AI2 by applying linear approximation, and thereby be able to handle larger DNNs with over 88K neurons.
%	& Low precision  when dealing with large input perturbation due to very coarse interval generated during the feedforward simulation. & \checkmark 
	& \textcolor{red}{Not Specified}
	& \checkmark	& \checkmark			& \checkmark		 & -- \\ \hline
\refstepcounter{rownumber}\therownumber & Wang \textit{et al.}, 2018~\cite{wang2018formal} 		\newline  \textsc{ReluVal}		
	& Proposes a symbolic interval analysis to estimate bounds of a neuron output with iterative refinement by bisecting the input range according to the order of sensitivity. It proclaims to work around 200x faster than the Reluplex.
%	& Suffering from low precision and high false positive rate when dealing with larger networks. & \checkmark
	& Not Specified (written in C)%~\footnote{\url{https://github.com/tcwangshiqi-columbia/ReluVal}}
	& \checkmark	& --	& -- 	 & -- \\ \hline
\refstepcounter{rownumber}\therownumber & Wang \textit{et al.}, 2018	\cite{wang2018efficient} 	\newline  \textsc{Neurify}		
	& Integrates directed constraint refinement and state-of-the-art linear approximation techniques into symbolic interval analysis and adopts a MILP solver to reason the property specification. It achieves better overall performance than ReluVal, and be able to verify DNNs with over 10k hidden units. It also supports verification of $L_{1}$ norm specifications through solving quadratic constraints.
%	& Still has improvement spaces for a better scalability. & \checkmark
	& Tensorflow (conversion required)%~\footnote{\url{https://github.com/tcwangshiqi-columbia/Neurify}}
	& \checkmark	& --	& -- & --\\ \hline
\refstepcounter{rownumber}\therownumber & Weng \textit{et al.}, 2018	\cite{weng2018towards} 		\newline  \textsc{Fast-Lin}, \textsc{Fast-Lip}		
	& Proposes a layer-wise linear approximation to estimate the bounds of ReLU output, and another estimation by bounding the local Lipschitz constant. Achieves two orders of magnitude faster than existing approaches that rely on SAT/LP encoding.
%	& Works on MLPs only and it is unsound for floating point arithmetic. & \checkmark
	& Tensorflow%~\footnote{\url{https://github.com/huanzhang12/CertifiedReLURobustness}}
	& \checkmark	& --	& -- & --\\ \hline
\refstepcounter{rownumber}\therownumber & Xiang \textit{et al.}, 2018~\cite{xiang2018output} 		\newline  \unofficialname{MaxSensitivity}						
	& Proposes a simulation based approach with provable soundness by interval arithmetic analysis and estimates the range of neurons' output.
%	& Poor scalability due to the coarse interval. & -- 
	& MATLAB
	& \checkmark	& \checkmark		& \checkmark		 	& --\\ \hline
\refstepcounter{rownumber}\therownumber & Zhang \textit{et al.}, 2018~\cite{zhang2018efficient} 	\newline  \textsc{CROWN}		
	& The first work that proposes a generic linear relaxation method for general activation functions to estimate bounds of a DNN output within polynomial time. The experiment shows it can handle DNNs with up to 10K neurons.
%	& No obvious issues. & \checkmark
	& Tensorflow%~\footnote{\url{https://github.com/crown-robustness/crown}}
	& \checkmark	& \checkmark			& \checkmark & --\\ \hline
\refstepcounter{rownumber}\therownumber & Bunel \textit{et al.}, 2018~\cite{bunel2018unified}		\newline  \textsc{BaB, BaBSB \& reluBaB}
	& Encompasses existing methods including Reluplex and Planet into a unified framework that performs branch-and-bound strategy to solve the optimization problem. Proposes interval refinement with higher precision and a reduced search space.
	& PyTorch %\footnote{\url{https://github.com/oval-group/PLNN-verification}}
	& & & & \\ \hline

\refstepcounter{rownumber}\therownumber & Katz \textit{et al.}, 2019	\cite{katz2019marabou}		\newline  \textsc{Marabou}		
	& Extends the Reluplex algorithm into a framework that accepts arbitrary DNNs with piecewise linear activation, and improves performance by implementing a new simplex core to replace the external solver in Reluplex. 
%	& Scalability is not evaluated in general way since the benchmarking is performed on ACAS Xu models only. & \checkmark
	& Tensorflow%~\footnote{\url{https://github.com/NeuralNetworkVerification/Marabou}}
	& \checkmark & --	& -- 	& \checkmark\\ \hline
\refstepcounter{rownumber}\therownumber & Tjeng \textit{et al.}, 2019~\cite{tjeng2019evaluating}	\newline  \textsc{MIPVerify}	
	& Proposes an MILP based encoding with \emph{progressive bounds tightening} applied during the reasoning stage, and thereby achieves a scalable \& complete verification that can handle DNNs with over 100K neurons.
%	& No obvious issue excepts no supports of activation other than ReLU. & \checkmark
	& Julia %\footnote{\url{https://github.com/vtjeng/MIPVerify.jl}}
	& \checkmark & --	& -- 	& \checkmark \\ \hline
\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2019~\cite{singh2019abstract} 	\newline  \textsc{DeepPoly}		
	& Proposes a more complicated polyhedral abstract domain to achieve higher precision in abstract interpretation, and it is also the first work that takes image rotation into account for the robustness verification.
%	& Still suffers from low precision concern when dealing with large neural network. & \checkmark
	& \textcolor{red}{Not Specified}
	& \checkmark	& \checkmark & \checkmark		 & --\\ \hline
\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2019~\cite{singh2019boosting}		\newline  \textsc{RefineZono}	
	& Introduces a heuristic bounds refinement by MILP solver after over-approximating neurons' output at each hidden layer, and thereby achieves a  better precision.
%	& Takes only ReLU activation into account and does not scale well when compared with other incomplete approaches. & \checkmark
	& \textcolor{red}{Not Specified}
	& \checkmark	& --	& -- & --\\ \hline
\refstepcounter{rownumber}\therownumber & Singh \textit{et al.}, 2019~\cite{singh2019beyond}		\newline  \textsc{kPoly} (aka. \textsc{RefinePoly})		
	& Proposes a finer approximation than DeepPoly called k-ReLU that jointly evaluates the output of multiple ReLU outputs within tha same layer.
%	& No obvious issues as an improvement work except missing support of activation other than ReLU. & \checkmark
	& \textcolor{red}{Not Specified}
	& \checkmark	& --	& -- & --\\ \hline
\refstepcounter{rownumber}\therownumber & Yisrael \textit{et al.}, 2019~\cite{yisrael2019abstraction} 	\newline  \unofficialname{CEGAR-Marabou}					
	& The first work that proposes abstract interpretation by simplifying the DNN architecture, that firstly reduces the number of neuron per layer to at most 4, and then iteratively refines the abstraction until achieving a successful verification.
%	& Comes with an sssumption that bias parameters are trivial and set to 0. Lack of comparable benchmarking with other abstraction-based works. & \checkmark
	& Not released
	& \checkmark	& --		&  --	& --\\ \hline

\refstepcounter{rownumber}\therownumber & Xiang \textit{et al.}, 2020~\cite{xiang2020reachable} 	\newline  \textsc{IGNNV}					
	& Proposes a simulation-based reachability analysis to verify safety properties by discretizing the input set into a finite number of intervals, and overapproximating the computation within the hidden layers. 
	%The verification is achieved by checking the existence of intersections between the estimated reachable set and unsafe regions. 
	It performs 30x faster than the former work \textsc{MaxSensitivity}.
	& MATLAB%\footnote{\url{https://github.com/xiangweiming/ignnv}}
	& \checkmark	& \checkmark		&  \checkmark	& --\\ \hline


		\end{longtable}
		% GRAND TABLE ENDS HERE
		\vspace{-5px}
		
		\textsuperscript{*} The name of tool has not been explicitly defined in the given literature, but are taken from the source code released, or commonly addressed in subsequent research. The name is usually cited from the function name or the paper title.
		\vspace{5pt}
		
		\textsuperscript{$\dagger$} We discuss the top three commonly used activation functions in this table. The checkmark symbol (\checkmark) denotes the corresponding activation function is supported in the given work, and conversely (--) means the given work does not accept such activation function. 
		\vspace{5pt}
		
		\textsuperscript{$\ddagger$} We identify a verification approach to be ``complete'' only if it does not allow false positive instances. The checkmark symbol (\checkmark) indicates the work achieves completeness on the basis of a sound verification, otherwise shown as (--). 
		\vspace{5pt}
		
		\textsuperscript{$\S$} That work is partially complete. Its completeness is guaranteed in verifying neural networks with ReLU functions only, but not applicable to arctan activation. We mark it complete since verifying arctan activation is not covered in the scope of this survey.
		
		%\begin{center}
		%	\textbf{End of table}
		%\end{center}
		
	\end{landscape}
	\twocolumn
} % end of scope of "\afterpage" directive

